Learning Union of Integer Hypercubes with Queries (Technical Report)

We study the problem of learning a finite union of integer (axis-aligned) hypercubes over the d-dimensional integer lattice, i.e., whose edges are parallel to the coordinate axes. This is a natural generalization of the classic problem in the computational learning theory of learning rectangles. We provide a learning algorithm with access to a minimally adequate teacher (i.e. membership and equivalence oracles) that solves this problem in polynomial-time, for any fixed dimension d. Over a non-fixed dimension, the problem subsumes the problem of learning DNF boolean formulas, a central open problem in the field. We have also provided extensions to handle infinite hypercubes in the union, as well as showing how subset queries could improve the performance of the learning algorithm in practice. Our problem has a natural application to the problem of monadic decomposition of quantifier-free integer linear arithmetic formulas, which has been actively studied in recent years. In particular, a finite union of integer hypercubes correspond to a finite disjunction of monadic predicates over integer linear arithmetic (without modulo constraints). Our experiments suggest that our learning algorithms substantially outperform the existing algorithms.

==> artifact-abstract.tex <==
%!TEX root = artifact-main.tex

We study the problem of learning a finite union of integer 
(axis-aligned) hypercubes over the $d$-dimensional integer lattice, i.e.,
whose edges are parallel to the coordinate axes. This is a natural
generalization of the classic problem in the computational learning theory of 
learning rectangles.
 We provide a learning algorithm with access to
a minimally adequate teacher (i.e. membership and equivalence oracles) that 
solves this problem in polynomial-time,
for any fixed dimension $d$. Over a non-fixed dimension, the problem subsumes
the problem of learning DNF boolean formulas, a central open problem in the
field. 
We have also provided extensions to handle infinite hypercubes in the union,
as well as showing how subset queries could improve the performance of the
learning algorithm in practice.
%We have also shown that the learning algorithm could be extended
%With the help of inclusion oracles, we provide a learning algorithm for the
%problem that runs in time polynomial also in $d$.
%be at least as hard as learning DNF with membership and equivalence queries, 
%for which the existence of a polynomial-time algorithm is a long-standing open 
%problem.
Our problem has a natural application to the problem of monadic 
decomposition of quantifier-free integer linear arithmetic formulas,
%SMT formulas (in particular, over integer linear arithmetic), 
which has been actively studied in recent years. In particular, a finite union
of integer hypercubes correspond to a finite disjunction of monadic
predicates over integer linear arithmetic (without modulos constraints). 
Our experiments suggest that our learning algorithms substantially outperform 
the existing algorithms.
 %over formulas that admit such 
%monadic decompositions.



